Task-Oriented Edge-Assisted Cooperative Data Compression, Communications and Computing for UGV-Enhanced Warehouse Logistics

This paper explores the growing need for task-oriented communications in warehouse logistics, where traditional communication Key Performance Indicators (KPIs)-such as latency, reliability, and throughput-often do not fully meet task requirements. As the complexity of data flow management in large-scale device networks increases, there is also a pressing need for innovative cross-system designs that balance data compression, communication, and computation. To address these challenges, we propose a task-oriented, edge-assisted framework for cooperative data compression, communication, and computing in Unmanned Ground Vehicle (UGV)-enhanced warehouse logistics. In this framework, two UGVs collaborate to transport cargo, with control functions-navigation for the front UGV and following/conveyance for the rear UGV-offloaded to the edge server to accommodate their limited on-board computing resources. We develop a Deep Reinforcement Learning (DRL)-based two-stage point cloud data compression algorithm that dynamically and collaboratively adjusts compression ratios according to task requirements, significantly reducing communication overhead. System-level simulations of our UGV logistics prototype demonstrate the framework's effectiveness and its potential for swift real-world implementation.

==> Algrithm/alg_cvae_train.tex <==
\begin{algorithm}[t]
\caption{TSCC Training Algorithm}
% This label should be put after caption
\label{alg_cvae_train}
\begin{algorithmic}[1]
\Statex \textbf{Initialization}: Initialize the neural network parameters $\alpha$ and $\delta$.

\State \textbf{Input}: Image dataset $\mathcal{X}$ with corresponding ground-truth agent output $\mathcal{A}$ and state information $\mathcal{M}$. 

\While{not converged}
    \State Sample $\bm{a}$ from $\mathcal{A}$ with the corresponding $\bm{m}$ from $\mathcal{M}$.
    \State Sample $\bm{x}$ from $\mathcal{X}$ according to $\bm{a}$ and $\bm{m}$.
    \State Encode image $\bm{x}$ to mean and standard deviation: 
    \Statex \quad \, $\bm{\mu}, \bm{\sigma} \leftarrow \mathrm{T}_{\alpha}(\bm{x})$.
    \State Sample latent vector using the \textit{reparameterization}
    \Statex \quad \, \textit{trick}: $\check{\bm{z}} \leftarrow \bm{\epsilon}\odot \bm{\sigma} + \bm{\mu}$.
    \State Reshape and normalize latent vector: $\tilde{\bm{z}} \leftarrow \mathrm{N}(\mathrm{F}(\check{\bm{z}}))$.
    \State Reconstruct image from $\tilde{\bm{z}}$: 
    \Statex \quad \, $\bm{y} \leftarrow \mathrm{T}^{-1}_\delta(\mathrm{F}^{-1}(\tilde{\bm{z}}))$.
    \State Generate control commands: $\hat{\bm{a}} \leftarrow \mathrm{A}_{\psi}(\bm{y}, \bm{m})$.
    \State Compute $\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta)$ and $\mathcal{L}_{\text{c-KL}}(\bm{a}, \bm{m}; \alpha)$.
    \State Update neural network parameters:
    \Statex \quad \, $\alpha \overset{+}{\leftarrow} -\nabla_{\alpha} (\beta_{\text{c-rec}}\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta) + \mathcal{L}_{\text{c-KL}}(\bm{a}, \bm{m}; \alpha))$.
    \Statex \quad \, $\delta  \overset{+}{\leftarrow} -\nabla_{\delta}\beta_{\text{c-rec}}\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta)$.
    
\EndWhile
\State \textbf{Output}: The coding neural network $\mathrm{T}_{\alpha}(\cdot)$ and $\mathrm{T}_{\delta}^{-1}(\cdot)$.
\end{algorithmic}
\end{algorithm}


==> Algrithm/alg_cvae_train_v1.0.tex <==
\begin{algorithm}[t]
\caption{TSCC Training Algorithm}
% This label should be put after caption
\label{alg_cvae_train}
\begin{algorithmic}[1]
\Statex \textbf{Initialization}: Initialize the neural network parameters $\alpha$ and $\delta$.

\State \textbf{Input}: Image dataset $\mathcal{X}$ with corresponding ground-truth agent output $\mathcal{A}$ and state information $\mathcal{M}$. 

\While{not converged}
    \State $\bm{a}, \bm{m} \leftarrow$ Random mini batch from ground truth 
    \Statex \quad \; $\mathcal{A}$ with corresponding state information $\mathcal{M}$.
    \State $\bm{x} \leftarrow$ Mini batch from image dataset $\mathcal{X}$ according to 
    \Statex \quad \; $\bm{a}, \bm{m}$.
    \State $\bm{\mu}, \bm{\sigma} \leftarrow \mathrm{T}_{\alpha}(\bm{x})$.
    \State $\bm{z} \leftarrow \mathrm{F}(\mathrm{N}(\mathrm{R}(\bm{\sigma}, \bm{\mu})))$.
    \State $\bm{y} \leftarrow \mathrm{T}^{-1}_\delta(\mathrm{F}^{-1}(\hat{\bm{z}}))$.
    \State $\hat{\bm{a}} \leftarrow \mathrm{A}_{\psi}(\bm{y}, \bm{m})$.
    \State $\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta) \leftarrow \mathbb{E}_{\bm{z} \sim q_{\alpha}(\bm{z} \mid \bm{a}, \bm{m})}[-\ln p_{\delta}(\bm{a} | \bm{m}, \bm{z})]$.
    \State $\mathcal{L}_{\text{c-KL}}(\bm{a}, \bm{m}; \alpha) \leftarrow \mathbb{E}_{\bm{z} \sim q_{\alpha}(\bm{z} \mid \bm{a}, \bm{m})}\left[\ln{\frac{q_{\alpha}(\bm{z} \mid \bm{a}, \bm{m})}{p(\bm{z} \mid \bm{m})}}\right]$.
    \State $\alpha \overset{+}{\leftarrow} -\nabla_{\alpha} (\beta_{\text{c-rec}}\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta) + \mathcal{L}_{\text{c-KL}}(\bm{a}, \bm{m}; \alpha))$.
    \State $\delta  \overset{+}{\leftarrow} -\nabla_{\delta}\beta_{\text{c-rec}}\mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta)$.
    
\EndWhile
\State \textbf{Output}: The coding neural network $\mathrm{T}_{\alpha}(\cdot)$ and $\mathrm{T}_{\delta}^{-1}(\cdot)$.
\end{algorithmic}
\end{algorithm}

==> Draft/1_0_intro.tex <==
\section{Introduction}
Edge computing enabled autonomous driving imposes extremely stringent requirements on traditional communication: 1) high computational demands: autonomous vehicles generate a vast amount of sensor data, including LiDAR, radar, camera, and GPS data, which must be transmitted and processed in real-time to enable safe and efficient driving. These high data volumes and stringent latency requirements pose a significant challenge for edge computing systems \cite{Liu_2019_edge}; 2) real-time responsiveness and latency requirements: edge computing systems must minimize the processing time required for sensor data analysis and decision-making, ensuring that the vehicle can respond to changing situations in a timely and accurate manner \cite{Liu_2019_edge}; 3) data exchange: edge computing systems must facilitate seamless communication and data exchange between entities, such as other vehicles, infrastructures, and cloud-based services, ensuring that the vehicle has access to the information it needs to make informed decisions \cite{Ameen_2019_deep}. The high mobility of vehicles greatly challenges traditional communications, especially when bandwidth is limited and with strong noise interference. Specifically, with the degradation of \gls{snr} of the communication channel, traditional communication suffers from sudden breaking down of performance, known as \textit{cliff effect}. 
%Edge computing enabled autonomous driving imposes extremely stringent communication requirements: 1) Transmitting multimedia, including images and point cloud data \cite{Li_2020_joint}, can consume a large amount of communication resource overhead. 2) Autonomous vehicles should make correct motion decisions in a very short time to respond to various unexpected situations, which requires communications to provide ultra-low latency services~\cite{She_2021_tutorial}. 3) Even small errors in self-driving can cause serious consequences~\cite{kiran2021deep}, which poses extremely high reliability requirements for communication reliability. 
%Fine-grained KPIs for motion control have been released in~\cite{3GPP}, where the use case for motion control requires communications to provide 99.9999 \% availability and 1ms cycle time. 
%However, the communication demands for the self-driving scenario are still unclear. Even worse, the overall performance of self-driving depends not only on communications, but also on different subsystems, including data sensing, compression, and control \cite{Wu_2022_TCP}. Therefore, designing self-driving from a task-oriented cross-system perspective shows the superiority compared to design communications system independently.

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.95\linewidth]{Figure/general_idea.pdf}
    \end{center}
       \caption{Draft figure for paper writing, needs to be improved in details.}
    \label{fig_general_idea}
\end{figure}

Semantic communication is seen as the most promising technology for 6G, with the aim of exploiting the semantics of transmitted data in order to push the Shannon limit and thus achieve higher utilization of communication resources. It is expected to fundamentally disrupt the existing communication architecture by considering the entire transmission process as a whole, rather than considering each subsegment in isolation~\cite{Chaccour_2022_less}. This is represented by a series of work based on AI-powered~\gls{jscc}, where the semantic similarity metric is successfully applied to different tasks, including the transmission of natural language~\cite{Xie_2021_deep}, images~\cite{Bourtsoulatze_2019_deep}, videos~\cite{Wang_2023_wireless}, and point cloud data~\cite{Shao_2021_branchy}, where \Gls{jscc} shows resilience to the \textit{cliff effect}, and outperforms separate source channel coding at lower \gls{snr}. However, current research mainly focuses on the data itself, such as the \gls{psnr} and \gls{msssim} index \cite{} of the images, or on some basic tasks, such as image classification \cite{Zhang_2023_deep}. Comprehensive tasks that can truly unlock the potential of transmitting data via \gls{jscc} have not yet received much attention.

We propose a task-oriented deep \gls{jscc} based on \gls{vae} to empower edge-enabled \gls{e2e} autonomous driving. Inspired by \gls{jscc} enabled image transmission \cite{} and the combination of \gls{jscc} and \gls{vae} \cite{}, we jointly consider data transmission and pragmatic tasks to design an \gls{e2e} communication with strong resistance to \gls{awgn}. In the perspective of task-oriented design, we exploit \gls{e2e} autonomous driving agent as the communication metric to train deep \gls{jscc}. Instead of viewing the source-channel codec as \gls{vae}, we jointly design \gls{vae} combining the autonomous driving agent. \Gls{awgn} is discussed in this work and shows the advantage of our proposed method. Generally, the major contributions of this work are summary as follows:
\begin{itemize}
    \item To the best of our knowledge, we are the first to explore the deep \gls{jscc} design for autonomous driving, which shed light on the potential of deep \gls{jscc} design for the comprehensive pragmatic task.
    \item We propose to extend the \glspl{vae} design to jointly consider the autonomous driving agent and source-channel codec.
    \item We deploy our model in the edge-enabled state-of-the-art \gls{e2e} autonomous driving agent to show the general case for \gls{e2e} learning framework. Our methodology shows significant performance improvement in terms of driving score over traditional communication and the previous \gls{jscc} method.
\end{itemize}

==> Draft/2_0_related_work.tex <==
\section{Related Work}
The rapid evolution of deep learning inspires novel communication designs to approach or even exceed the Shannon limit. Semantic communication \cite{Chaccour_2022_less, Yang_2023_semantic, Qin_2022_semantic} is one promising direction that shifts the focus from the transmitted bits to the meaning carried by the transmitted bits. In particular, the deep \gls{jscc} design shows strong capability under limited bandwidth and noise inference to achieve satisfactory performance of tasks compared to traditional communication. Using semantic communication, text can be transmitted without enforcing the guarantee that all words or even sentences are transmitted correctly, while received text can still convey similar meanings \cite{Xie_2021_deep, Farsad_2018_deep}. In addition, \cite{Kurka_2019_seccessive, Bourtsoulatze_2019_deep, Kurka_2020_deepJSCC} proposed deep \glspl{jscc} for wireless image transmission and outperform separate traditional source coding (e.g. JPEG and JPEG2000) and channel coding (e.g. LDPC). \cite{Tung_2022_deepJSCC} design a ﬁnite channel input state to adopt deep \gls{jscc} on common hardware, which showed the possibility of \gls{jscc} empowered edge computing. However, the training of deep \gls{jscc} is generally closely related to the \gls{snr} of the channel itself, and it is generally necessary to train different models for channels with different \gls{snr}. \cite{Saidutta_2021_joint} introduced \gls{vae} in the design of a deep \gls{jscc}, which shows a better generalization for channels with different \gls{snr}. However, current work has mainly focused on basic tasks， such as image classification \cite{Zhang_2023_deep}. 

% Edge computing for autonomous driving, the challenges can be solved by JSCC
Autonomous driving requires storing and processing massive amounts of data generated by sensors and V2X communication, which challenges on-board processing and cloud computing in terms of power constraints and communication latency, respectively \cite{Zhang_2020_mobile}. Edge computing in autonomous driving is crucial to handle real-time data processing and decision-making requirements \cite{Liu_2019_edge}. Combining edge computing, deep \gls{jscc}, and \gls{e2e} autonomous driving agent \cite{Wu_2022_TCP} is promising to achieve semantic communication by task-oriented design. This synergy could facilitate real-time analytics of extensive sensor data (LiDAR, camera, radar), sheding light on the future direction.

% Our work
The current literature indicates a gap in the application of deep \gls{jscc} in the context of edge computing for autonomous driving. Our research aims to bridge this gap by demonstrating how a deep \gls{jscc} framework can improve the efficiency and reliability of data communication in autonomous vehicles. This approach not only reduces the data rate but also ensures the robustness of the communication under varying channel conditions. This exploration is critical to realize the full potential of autonomous vehicles in real-world scenarios.


==> Draft/3_0_system_model.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.9\linewidth]{Figure/case_study.pdf}
    \end{center}
       \caption{Draft figure for describing the framework.}
    \label{fig_case_study}
\end{figure*}
\section{System Model}
The proposed self-driving scenario is shown in \cref{fig_general_idea}. This involves equipping an automated vehicle with a variety of sensors, such as an RGB camera, depth camera, lidar, radar, and speedometer. These instruments work together to collect comprehensive data from the environment as well as the vehicle's own operational metrics.

The collected data are then encoded and transmitted via \gls{rf} to a proximal edge server strategically located near a base station. The edge server, acting as a computational hub, is tasked with processing the received data using the deployed autonomous driving agent.

After interpreting the incoming data, the agent immediately generates control commands tailored to the vehicle's current scenario and operational needs. These control commands are then sent back to the automated vehicle, enabling it to take the necessary driving actions in a timely manner. This efficient closed-loop communication and control system provides the automated vehicle with the agility and precision required for safe and reliable autonomous driving.

Within our autonomous driving scenario, there are several potential issues and areas of research. These include factors such as time delay, jitter, and queueing, all of which could significantly impact the performance and effectiveness of the communication system in real-world applications. Despite the importance of these issues, in this work, we focus on the challenge of bandwidth utilization and data transmission efficiency, with an emphasis on image data, since images captured by vehicle cameras are the primary source of information about the vehicle's environment, and effective compression and transmission of these data are critical to the safety and performance of the autonomous driving system.

Raw sensor data, such as high-resolution images, consumes a large amount of bandwidth during transmission. Traditionally, data compression in communication systems is achieved through source coding, which includes methods such as quantization \cite{}, entropy coding \cite{}, and lossy compression algorithms \cite{}. These traditional methods aim to minimize the average bit rate of a given source at a given level of distortion. However, they often ignore the underlying semantics of the data, leading to poor data reconstruction and interpretation, even achieving a low \gls{ber}, especially at low \gls{snr}.

Semantic-based compression methods learn a representation to compress the data that captures the most semantically relevant features. The advantage of this method is that it is more robust to transmission errors in low \gls{snr} scenarios. Even if some bits are corrupted during transmission, the overall semantic meaning of the data can still be preserved. 

However, for complex mission-critical systems, such as self-driving vehicles, simply considering the semantics of the data may not be sufficient. Therefore, we propose to move beyond semantic communications to task-oriented communications. This new paradigm focuses on the ultimate goal or task that the communication system serves. It considers not only the semantics of the data, but also the specific task requirements and goals of the autonomous driving system. This task-oriented communication can further enhance the effectiveness of the communication system, potentially leading to even better performance under challenging conditions compared to traditional and semantic-based methods.

In the following sections, we present a case study that illustrates the implementation and effectiveness of our proposed design for edge-assisted autonomous driving. Next, we demonstrate the loss function and the training process. Especially, an \gls{e2e} self-driving framework based on a monocular RGB camera is used as a baseline. This case study serves as a tangible representation of the theoretical principles presented in the previous sections and provides an application-oriented perspective to our research. \Cref{fig_case_study} shows the implementation of our proposed case study.

\subsection{\gls{vae}}
Previous works \cite{Xie_2021_deep, Weng_2021_semantic} have designed the \gls{e2e} training of the \gls{dnn}-based source and channel coding in an autoencoder way. In contrast, we design the source and channel coding based on \gls{vae} \cite{}. \glspl{vae} are a class of generative models that leverage the power of neural networks for the encoding and decoding process while incorporating a probability distribution for data generation and latent space modeling. 

The basic idea behind VAEs lies in their structure, which consists of an encoder neural network, a latent space, and a decoder neural network. Given an input data sample $\bm{x}$, the encoder neural network $p_{\theta}(\bm{z}\mid \bm{x})$ maps it to a distribution over the latent space, where a vector $\bm{z}$ in the latent space is typically imposed a prior $\bm{z} \sim \mathcal{N}(\bm{0}, \mathbf{I})$. The parameters of this distribution, mean $\bm{\mu}$ and standard deviation $\bm{\sigma}$, are output by the encoder. A latent vector $\bm{z}$ is then sampled by \textit{reparameterization trick} to maintain the differentiability, which is essential for backpropagation during training.

This sampled latent vector $\bm{z}$ is fed into the decoder neural network $q_{\phi}(\bm{x}\mid \bm{z})$, which attempts to reconstruct the original data sample $\bm{x}$. The overall objective of \gls{vae} is to minimize the following loss function
\begin{align}
\mathcal{L}_\text{VAE}
    = & -\text{ELBO}(\bm{x}) \label{eq_loss_vae_1}\\
    = & \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x})}\left[-\ln p_{\theta}(\bm{x} \mid \bm{z})\right] + \mathrm{KL}(q_{\phi}(\bm{z} \mid \bm{x}) \| p(\bm{z}))  \label{eq_loss_vae_2}\\
    = & \mathcal{L}_{\text{rec}} + \mathcal{L}_{\text{KL}} \label{eq_loss_vae_3},
\end{align}
where $\theta$ and $\phi$ are the parameters for the encoder neural network and decoder neural network, respectively. KL represents \gls{kl} divergence.

Specially, $\mathcal{L}_{\text{rec}}$ is equivalent to \gls{mse} between the original data point and the mean of $p_{\theta}(\bm{x} \mid \bm{z})$, which in this case is the reconstructed data sample $\hat{\bm{x}}$
\begin{equation}
    \mathcal{L}_\text{rec}(\bm{x}, \hat{\bm{x}}) = \text{MSE}(\bm{x}, \hat{\bm{x}}). \label{eq_loss_vae_mse}
\end{equation}
Since $q_{\phi}(\bm{x}\mid \bm{z}) = \mathcal{N}(\bm{\mu}, \bm{\sigma})$ and $\bm{z} \sim \mathcal{N}(\bm{0}, \mathbf{I})$, $\mathcal{L}_{\text{KL}}$ can be rewrite as
\begin{equation}
    \mathcal{L}_{\text{KL}}(\bm{\mu}, \bm{\sigma}) = \frac{1}{2}\sum(\bm{\mu}^{2}+\bm{\sigma}^{2} - \ln\bm{\sigma}^{2} - 1). \label{eq_loss_vae_kl}
\end{equation}
Specially, $\beta$-\gls{vae} \cite{beta_VAE} extended the loss function of vanilla \gls{vae} by adding an coefficient $\lambda_{\mathrm{beta}}$
\begin{equation}
    \mathcal{L}_\text{VAE}
    = \mathcal{L}_{\text{rec}} + \lambda_{\mathrm{beta}}\mathcal{L}_{\text{KL}}
    \label{eq_loss_betaVAE}
\end{equation}


\subsection{Onboard Image Processing}
\label{subsec_sysMod_framework}
The input RGB image from CARLA can be denoted as $\bm{x} \in \mathbb{R}^{3\times H \times W}$, where $3$ is the number of channels,  $H$ and $W$ are the height and width of the image in the number of pixels, respectively. 



On the vehicle side, the RGB image is first encoded by a task encoder
\begin{equation}
    (\bm{\mu}_{\mathrm{T}}, \bm{\sigma}_{\mathrm{T}}) = \mathrm{T}_\alpha(\bm{x}),
    \label{eq_task_encoder}
\end{equation}
where $\mathrm{T}_\alpha(\cdot)$ is the task encoder with the parameters $\alpha$. $\bm{\mu}_{\mathrm{T}} \in \mathbb{R}^{1\times d_{\mathrm{T}}}$ and $\bm{\sigma}_{\mathrm{T}} \in \mathbb{R}^{1\times d_{\mathrm{T}}}$ are the mean and standard deviation of the normal distribution, respectively. The task features $\bm{z}_{\mathrm{T}} \in \mathbb{R}^{1\times d_{\mathrm{T}}}$ can be sample by \textit{reparameterization trick}
\begin{equation}
    \bm{z}_{\mathrm{T}} = \bm{\epsilon}_{\mathrm{T}}\odot \bm{\sigma}_{\mathrm{T}} + \bm{\mu}_{\mathrm{T}},
\end{equation}
where $\bm{\epsilon}_{\mathrm{T}} \in \mathbb{R}^{1\times d_{\mathrm{T}}}$ is sample from $\mathcal{N}(\bm{0}, \mathbf{I})$, $d_{\mathrm{T}}$ is the dimension of the task features $\bm{z}_\mathrm{T}$, $\odot$ represent elements wise multiplication.

The task features $\bm{z}_{\mathrm{T}}$ is then further encoded by a channel encoder $\mathrm{C}_{\beta}(\cdot)$ with parameters $\beta$
\begin{equation}
    (\bm{\mu}_{\mathrm{C}}, \bm{\sigma}_{\mathrm{C}}) = \mathrm{C}_\beta(\bm{z}_{\mathrm{T}}),
    \label{eq_channel_encoder}
\end{equation}
where $\bm{\mu}_{\mathrm{C}}$ and $\bm{\sigma}_{\mathrm{C}}$ are the mean and standard deviation of the normal distribution, respectively. The symbol stream $\bm{z}_{\mathrm{C}} \in \mathbb{R}^{1\times d_{\mathrm{C}}}$ can be obtained by reparameterization trick as
\begin{equation}
    \bm{z}_{\mathrm{C}} = \bm{\epsilon}_{\mathrm{C}}\odot \bm{\sigma}_{\mathrm{C}} + \bm{\mu}_{\mathrm{C}},
    \label{eq_reparam_channel}
\end{equation}
where $\bm{\epsilon}_{\mathrm{C}} \in \mathbb{R}^{1\times d_{\mathrm{C}}}$ is sample from $\mathcal{N}(\bm{0}, \mathbf{I})$, $d_{\mathrm{C}}$ is the dimension of the symbol stream $\bm{z}_{\mathrm{C}}$.

The transmission process through the channel layer can be modeled as 
\begin{equation}
    \hat{\bm{z}}_{\mathrm{C}} = \bm{h}\odot \bm{z}_{\mathrm{C}}+\bm{n},
    \label{eq_channel_layer}
\end{equation}
where the $\bm{h} \in \mathbb{R}^{1\times d_{\mathrm{C}}}$ represents the Rayleigh fading channel with $\mathcal{CN}(\bm{0}, \mathbf{I})$ and $\bm{n} \sim \mathcal{CN}(0, \sigma_{\mathrm{AWGN}}^{2}\mathbf{I})$. In addition, the \gls{awgn} channel can be represented as
\begin{equation}
    \hat{\bm{z}}_{\mathrm{C}} = \bm{z}_{\mathrm{C}}+\bm{n}.
\end{equation}
As shown in \cref{fig_case_study}, the task features $\hat{\bm{z}}_{\mathrm{T}}$ can be reverted from symbol stream $\hat{\bm{z}_{\mathrm{C}}}$
\begin{equation}
    \hat{\bm{z}}_{\mathrm{T}} = \mathrm{C}^{-1}_\gamma(\hat{\bm{z}}_{\mathrm{C}}),
    \label{eq_channel_decoder}
\end{equation}
where $\mathrm{C}^{-1}_\gamma(\cdot)$ is the channel encoder with the parameters $\gamma$. The reconstructed image $\hat{\bm{x}}$ can be recovered from task features $\hat{\bm{z}_{\mathrm{T}}}$
\begin{equation}
    \hat{\bm{x}} = \mathrm{T}^{-1}_\delta(\hat{\bm{z}}_{\mathrm{T}}),
    \label{eq_task_decoder}
\end{equation}
where $\mathrm{T}^{-1}_\delta(\cdot)$ is the task decoder with parameters $\delta$.

Since the goal of our task-oriented design is to maximize self-driving performance rather than to minimize the difference between $\bm{x}$ and $\hat{\bm{x}}$, this leads to the challenges of designing the loss function that preserves the most task-relevant information for the autonomous driving agent and takes driving performance into account as the optimization target.

Based on the \cref{eq_loss_vae_mse}, \cref{eq_loss_vae_kl}, \cref{eq_channel_encoder}, \cref{eq_reparam_channel}, and \cref{eq_channel_decoder} the loss function of the channel coding can be written as
\begin{equation}
    \mathcal{L}_{\mathrm{ch}}(\bm{z}_{\mathrm{T}}, \hat{\bm{z}}_{\mathrm{T}}, \bm{\mu}_{\mathrm{C}}, \bm{\sigma}_{\mathrm{C}})=\mathcal{L}_{\mathrm{rec}}(\bm{z}_{\mathrm{T}}, \hat{\bm{z}}_{\mathrm{T}}) + \mathcal{L}_{\mathrm{KL}}(\bm{\mu}_{\mathrm{C}}, \bm{\sigma}_{\mathrm{C}}),
\end{equation}
where $\mathcal{L}_{\mathrm{rec}}(\bm{z}_{\mathrm{T}}, \hat{\bm{z}}_{\mathrm{T}})$ can be regarded as semantic loss of the channel coding.

The loss function to train the task coding neural network is similar to the loss function of the channel coding neural network. However, we do not use $\mathrm{MSE}(\bm{x}, \hat{\bm{x}})$ as a loss of reconstruction. Instead, we use the discrepancy between the baseline agent output $\bm{a}$ and the $\hat{\bm{a}}$ generated by the reconstructed image $\hat{\bm{x}}$. The details are demonstrated in the following subsection.



==> Draft/3_1_system_model.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=1\linewidth]{Figure/case_study.pdf}
    \end{center}
       \caption{Framework of the deep \gls{jscc} enabled autonomous driving.}
    \label{fig_case_study}
\end{figure*}
\section{System Model}
The proposed edge-enabeld autonomous driving scenario is shown in \cref{fig_general_idea}. This involves equipping an automated vehicle with a variety of sensors, such as RGB cameras, depth cameras, LiDARs, radars, and speedometers. These instruments work together to collect comprehensive data from the environment, as well as the vehicle's own operational metrics.

These data are encoded and transmitted to a proximal edge server via wireless communication, where the edge server, located near a base station, acts as a computational hub. Here, the data are processed by an autonomous driving agent, which interprets the information and generates appropriate control commands for the vehicle's current scenario. These commands are transmitted back to the vehicle, allowing for precise and timely driving actions essential for safe autonomous driving.

In our scenario, we identify several challenges, including time delay, jitter, and queueing, which could impact the communication system's performance in real-world applications. Our focus, however, is on bandwidth utilization and data transmission efficiency, emphasizing image data. Images are crucial as they provide primary information about the vehicle's environment. Effective image compression and transmission are critical to the safety and performance of the autonomous driving system.

Traditional data compression methods in communication systems, such as quantization \cite{}, entropy coding \cite{}, and lossy compression algorithms \cite{}, aim to minimize bit rates at a certain distortion level. However, these methods often overlook the semantics of the data, leading to suboptimal task performance, particularly at low \glspl{snr}.

Semantic-based compression methods focus on capturing the most semantically relevant features of the data, offering robustness against transmission errors in low SNR scenarios. Nevertheless, for complex mission-critical systems like autonomous vehicles, considering data semantics alone may not suffice. Therefore, we propose a shift towards task-oriented communications, focusing on the end goal of the communication system and integrating the specific task requirements and goals of the autonomous driving system.

This task-oriented approach promises to enhance communication effectiveness, potentially outperforming traditional and semantic-based methods in challenging conditions. The following sections present a case study demonstrating our proposed design's implementation and effectiveness in edge-enabled autonomous driving. We demonstrate the loss function and the training process, using an \gls{e2e} autonomous driving framework based on a monocular RGB camera as a baseline. \Cref{fig_case_study} illustrates our case study implementation, providing a practical perspective on the theoretical concepts. In particular, our approach integrates \gls{jscc} within the edge computing framework to address the challenges of bandwidth constraint and data transmission efficiency. 

\subsection{Variational Autoencoder}
Previous works \cite{Xie_2021_deep, Weng_2021_semantic} have designed the \gls{e2e} training of \gls{dnn}-based \gls{jscc} in an autoencoder way. Inspired by \cite{Saidutta_2021_joint}, we designed the source channel codec based on \gls{vae}. Furthermore, our results show that the integration of vanilla \gls{vae} without further modification is noise-resistant in nature.

\glspl{vae} are a class of generative models that leverage the power of neural networks for the encoding and decoding process while incorporating a probability distribution for data generation and latent space modeling. 

The basic idea behind \glspl{vae} lies in their structure, which consists of an encoder neural network, a latent space, and a decoder neural network. Given an input data sample $\bm{x}$, the encoder neural network $p_{\theta}(\bm{z}\mid \bm{x})$ maps it to a distribution over the latent space, where a vector $\bm{z}$ in the latent space is typically imposed a prior $\bm{z} \sim \mathcal{N}(\bm{0}, \mathbf{I})$. The parameters of this distribution, mean $\bm{\mu}$ and standard deviation $\bm{\sigma}$, are output by the encoder. A latent vector $\bm{z}$ is then sampled by \textit{reparameterization trick} to maintain the differentiability, which is essential for backpropagation during training.

This sampled latent vector $\bm{z}$ is fed into the decoder neural network $q_{\phi}(\bm{x}\mid \bm{z})$, which attempts to reconstruct the original data sample $\bm{x}$. The overall objective of \gls{vae} is to minimize the following loss function
\begin{align}
\mathcal{L}_\text{VAE}
    = & -\text{ELBO}(\bm{x}) \label{eq_loss_vae_1}\\
    = & \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x})}\left[-\ln p_{\theta}(\bm{x} \mid \bm{z})\right] + \mathrm{KL}(q_{\phi}(\bm{z} \mid \bm{x}) \| p(\bm{z}))  \label{eq_loss_vae_2}\\
    = & \mathcal{L}_{\text{rec}} + \mathcal{L}_{\text{KL}} \label{eq_loss_vae_3},
\end{align}
where $\theta$ and $\phi$ are the parameters for the encoder neural network and decoder neural network, respectively. KL represents \gls{kl} divergence.

Specially, $\mathcal{L}_{\text{rec}}$ is equivalent to \gls{mse} between the original data point and the mean of $p_{\theta}(\bm{x} \mid \bm{z})$, which in this case is the reconstructed data sample $\hat{\bm{x}}$
\begin{equation}
    \mathcal{L}_\text{rec}(\bm{x}, \hat{\bm{x}}) = \text{MSE}(\bm{x}, \hat{\bm{x}}). \label{eq_loss_vae_mse}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Since $q_{\phi}(\bm{x}\mid \bm{z}) = \mathcal{N}(\bm{\mu}, \bm{\sigma})$ and $\bm{z} \sim \mathcal{N}(\bm{0}, \mathbf{I})$, $\mathcal{L}_{\text{KL}}$ can be rewrite as
\begin{equation}
    \mathcal{L}_{\text{KL}}(\bm{\mu}, \bm{\sigma}) = \frac{1}{2}\sum(\bm{\mu}^{2}+\bm{\sigma}^{2} - \ln\bm{\sigma}^{2} - 1). \label{eq_loss_vae_kl}
\end{equation}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\beta$-\gls{vae} \cite{beta_VAE} extended the loss function of vanilla \gls{vae} by adding an coefficient $\beta$
\begin{equation}
    \mathcal{L}_\text{VAE}
    = \beta_{\mathrm{rec}}\mathcal{L}_{\text{rec}} + \mathcal{L}_{\text{KL}},
    \label{eq_loss_betaVAE}
\end{equation}
where we use $\beta_{\mathrm{rec}}$ for $\mathcal{L}_{\mathrm{rec}}$ to control the training balance.

\Gls{cvae} introduce a class label $y$ as a condition, thus the new loss function can be extended from \cref{eq_loss_vae_2}
\begin{align}
    \mathcal{L}_{\mathrm{CVAE}} &= \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x}, \bm{y})}\left[-\ln p_{\theta}(\bm{x} \mid \bm{y}, \bm{z})\right] \notag \\ 
    & \ \ \ + \mathrm{KL}(q_{\phi}(\bm{z} \mid \bm{x}, \bm{y}) \| p(\bm{z} \mid \bm{y})) \\
    & = \mathcal{L}_{\text{c-rec}} + \mathcal{L}_{\text{c-KL}}
    \label{eq_loss_cvae}
\end{align}


\subsection{Onboard Image Processing}
\label{subsec_sysMod_framework}
The input RGB image can be denoted as $\bm{x} \in \mathbb{R}^{3\times H \times W}$, where $3$ is the number of channels,  $H$ and $W$ are the height and width of the image in the number of pixels, respectively. Specifically, we denote source bandwidth as $n=3\times H \times W$ \cite{Bourtsoulatze_2019_deep}.

On the vehicle side, instead of directly mapping RGB images to channel inputs \cite{}, the distributions of channel inputs are first derived
\begin{equation}
    (\bm{\mu}_{x}, \bm{\sigma}_{x}) = \mathrm{J}_\alpha(\bm{x}),
    \label{eq_task_encoder}
\end{equation}
where $\mathrm{J}_\alpha(\cdot)$ is the joint task encoder with the parameters $\alpha$. $\bm{\mu}_{x} \in \mathbb{R}^{d}$ and $\bm{\sigma}_{x} \in \mathbb{R}^{d}$ are the mean and standard deviation of the normal distribution, respectively. The channel inputs $\bm{z}_{x} \in \mathbb{C}^{k}$, where $k=\frac{d}{2}$, can be sampled by \textit{reparameterization trick}
\begin{align}
    \bm{z}_{x} &= \mathrm{F}(\mathrm{R}(\bm{\sigma}_{x}, \bm{\mu}_{x}))\\
    &= \mathrm{F}(\bm{\epsilon}\odot \bm{\sigma}_{x} + \bm{\mu}_{x}),
    \label{eq_reparam_reshape}
\end{align}
where $\bm{\epsilon} \in \mathbb{R}^{d}$ is sample from $\mathcal{N}(\bm{0}, \mathbf{I})$, $d$ is the dimension of the latent vector $\bm{z}_x$, $k$ is the channel bandwidth \cite{Bourtsoulatze_2019_deep}, $\odot$ represent elements wise multiplication, $\mathrm{R}$ denotes reparameterization trick, and $\mathrm{F}$ is the reshape function.

The transmission process through the channel layer can be modeled as 
\begin{equation}
    \hat{\bm{z}}_{x} = \bm{h}\odot \bm{z}_{x}+\bm{n},
    \label{eq_channel_layer}
\end{equation}
where the $\bm{h} \in \mathbb{C}^{k}$ represents the Rayleigh fading channel with $\mathcal{CN}(\bm{0}, \mathbf{I})$ and $\bm{n} \sim \mathcal{CN}(0, \bm{\sigma}_{\mathrm{awgn}}^{2}\mathbf{I})$. Specially, the \gls{awgn} channel can be represented as
\begin{equation}
    \hat{\bm{z}}_{x} = \bm{z}_{x}+\bm{n}.
\end{equation}

where $\hat{\bm{z}}_{\mathrm{T}}$ is received channel inputs. 
The reconstructed image $\hat{\bm{x}}$ can be recovered from received channel inputs
\begin{equation}
    \hat{\bm{x}} = \mathrm{J}^{-1}_\delta(\mathrm{F}^{-1}(\hat{\bm{z}}_{x})),
    \label{eq_task_decoder}
\end{equation}
where $\mathrm{J}^{-1}_\delta(\cdot)$ is the task decoder with parameters $\delta$, and $\mathrm{F}^{-1}$ is the inverse reshape function.

Since the goal of our task-oriented design is to maximize autonomous driving performance rather than to minimize the difference between $\bm{x}$ and $\hat{\bm{x}}$, this leads to the challenges of designing the loss function that preserves the most task-relevant information for the autonomous driving agent and takes driving performance into account as the optimization target.

Based on the \cref{eq_loss_vae_3}, the loss function of the \gls{jscc} can be written as
\begin{equation}
    \mathcal{L}_{\mathrm{VAE}}(\bm{x}, \hat{\bm{x}}, \bm{\mu}_{x}, \bm{\sigma}_{x})=\mathcal{L}_{\mathrm{rec}}(\bm{x}, \hat{\bm{x}}) + \mathcal{L}_{\mathrm{KL}}(\bm{\mu}_{x}, \bm{\sigma}_{x}),
    \label{loss_jscc_vae}
\end{equation}
where $\mathcal{L}_{\mathrm{rec}}(\bm{x}, \hat{\bm{x}})$ can be regarded as semantic loss.

However, \cref{loss_jscc_vae} overlooks task-relevant features, leading to suboptimal task performance. Dealing with that problem, we propose to use the discrepancy between the baseline agent output $\bm{a}$ and the $\hat{\bm{a}}$ generated by the reconstructed image $\hat{\bm{x}}$ as a reconstruction loss, instead of $\mathrm{MSE}(\bm{x}, \hat{\bm{x}})$. 

\subsection{Edge-Enabled Autonomous Driving Agent}
In order to generate control commands that best fit the current situation, autonomous driving requires not only information about the environment (e.g., RGB image), but also some additional information, such as navigation information and the current speed of the vehicle. As shown in \cref{fig_case_study}, the additional information, denoted as $m$, is sent by traditional communication. This is done for two reasons: 1) semantic communication may fail to preserve the fidelity of critical information, which requires strict similarity between input and output; 2) transmission of this additional information consumes far fewer communication resources compared with transmission of images; 3) as an initial research to explore the application of \gls{jscc} on edge-enabled autonomous diving, we first focus on image transmission. 

After receiving lossy additional information $\hat{m}$ and reconstructing the image $\hat{x}$, the edge-deployed autonomous driving agent generates control commands
\begin{equation}
    \hat{a} = \mathrm{A}(\hat{x}, \hat{m}),
\end{equation}
where $\mathrm{A}$ denotes the autonomous driving agent, $\hat{a}$ is the control commands generated from lossy information. 

\subsection{Training of Task-Oriented CVAE}
In the training of the proposed \gls{jscc} model, the noise channel is not considered, which means $z_x = \hat{z}_x$, $m = \hat{m}$. The baseline control commands $a$ are generated by lossless information. Assume that there is a mapping from $a$ to $x$, which can be denoted as $\mathrm{D}$, then the following relation can be satisfied
\begin{equation}
    \hat{a} = \mathrm{A}(\mathrm{J}^{-1}_\delta(\mathrm{F}^{-1}(\mathrm{F}(\mathrm{R}(\mathrm{J}_{\alpha}(\mathrm{D}(a)))))), \hat{m}).
    \label{eq_a2hata}
\end{equation}
In \cref{eq_a2hata}, additional information act as conditional vector for structure of \gls{cvae}. Thus, the task-oriented loss function can be obtained
\begin{equation}
    \mathcal{L}(\bm{a}, \hat{\bm{a}}, \bm{\mu}_{x}, \bm{\sigma}_{x})=\mathcal{L}_{\mathrm{c-rec}}(\bm{a}, \hat{\bm{a}}) + \mathcal{L}_{\mathrm{c-KL}}(\bm{\mu}_{x}, \bm{\sigma}_{x}).
\end{equation}
During training, the backpropagation stops at $x$.


Specially, it is not trivial to maintain the intact structure and parameters of the autonomous driving agent. With the least modification, the same autonomous driving agent can be deployed on both the edge and vehicle, which shows great potential for generalization.

==> Draft/4_0_result.tex <==
\section{Result}
\subsection{Dataset}
CARLA \cite{CARLA} is an open-source simulator for autonomous driving research, providing a rich, detailed, and highly realistic urban environment with a wide range of dynamic agents and traffic scenarios. CARLA enables us to test our design under varied and challenging conditions that closely mimic real-world driving situations.

% The number will be updated later
The image dataset built by \cite{Wu_2022_TCP} is used to train our neural network, which consists of images of the sizes $H=256$ and $W=900$. The training set contains about 196,000 images from 4 maps (Town01, Town03, Town04, and Town06), and the testing set contains 27,201 images from another 4 maps (Town02, Town05, Town07, and Town10). In addition to offline testing, we use Town02 and Town05 to test autonomous driving performance based on the proposed framework in simulation.

\subsection{Evaluation Metrics}
To evaluate the effectiveness of our approach, we conduct trials on the CARLA simulator and evaluate the driving score, a metric determined by the vehicle's ability to follow predetermined waypoints, reach the destination, and avoid violating traffic rules. The tests are carried out on eight routes from \textbf{Town02} and eight routes from \textbf{Town05}, with each route repeated three times for robustness. Driving performance can be evaluated in three aspects: route completion score, infraction score, and driving score\footnote{\url{https://leaderboard.carla.org/}}. The route completion score quantifies the ratio of completed road segments to the total planned distance; the infraction score takes into account any rule violations initiated by the autonomous agent; and the overall driving score, based on the previous two metrics, is an indicator of overall performance.

We compare our proposed framework with the classic image compression method, JPEG, JPEG2000, and BPG, followed by (2048, 6144) LDPC. In fairness, we configure these baselines to achieve an equivalent order of \textit{bandwidth compression ratio}. Although the compression rate of the traditional image compression method is not fixed, we calculate the average bandwidth ratio in the test set to configure each traditional image compression method. The average bandwidth compression ratios are 0.044, 0.021, and 0.019 for JPEG, JPEG2000, and BPG, respectively. Specially, for the coding neural network, we set $d=4096$, $k=2048$, so that the bandwidth compression ratio is 0.003. We intentionally configure the compression ratio of our model smaller than that of the traditional method, in order to show the advantages of our model under the low \gls{snr} condition.

To evaluate the performance of our proposed deep \gls{jscc} framework, we systematically varied \glspl{snr} by manipulating the noise variance $\sigma_{\mathrm{awgn}}^2$. We then compared the framework's performance to an upper bound on the performance of any digital transmission scheme that utilizes JPEG, JPEG2000, or BPG for source compression.

\subsection{Evaluation on CARLA}
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.95\linewidth]{Figure/results.pdf}
    \end{center}
       \caption{\textcolor{red}{The figure and data will be updated later.}}
    \label{fig_results}
\end{figure}



==> Table/tradi_metrics.tex <==
\begin{table}
\caption{Human Perceptional metrics}
\label{tab_tradi_metrics}
\begin{center}
\begin{tabular}{cccc}
\toprule
Method & PSNR(dB) $\uparrow$& MS-SSIM $\uparrow$& FID$\downarrow$\\
\midrule
    JPEG & 34.56 & 0.99 & 5.83\\ 
    JPEG2000 & 37.54 & 0.99 & 7.17 \\
    BPG & 34.93 & 0.98 & 6.68 \\
    JSCC-AE & 19.74 & 0.56 & 173.46 \\
    JSCC-VAE  & 20.85 & 0.66 & 160.66 \\
    TSCC & 7.72 & 0.13 & 347.30 \\
\bottomrule
\end{tabular}
\end{center}
\bigskip

\end{table}

==> _old/1_intro.tex <==
\section{Introduction}


% Some high-level introduction
As the era of intelligent transportation systems approaches, the concept of autonomous driving has moved from a futuristic vision to an imminent reality. The integration of advanced communication systems with automotive technology is leading the development of connected automation systems, such as autonomous driving. Edge computing brings computing and data storage closer to where they are needed, reducing latency, saving computational overhead, and saving bandwidth. The need for edge-enabled autonomous driving is driven by the limitations of traditional cloud computing models, which struggle to meet the real-time, high-bandwidth demands of autonomous vehicles.

Edge-enabled autonomous driving presents formidable challenges to traditional communication systems. Key challenges include: 
%\textcolor{blue}{you may discuss from high data throughput, low latency and reliability, computing, and implicit that the importance of your work and ready to solve them, therefore highlight your contributions}
\begin{enumerate}
    \item \textit{High Computational Overhead}: Autonomous vehicles generate a substantial amount of sensor data (e.g., radar, camera, and GPS), necessitating real-time transmission and processing for safe and efficient driving \cite{Liu_2019_edge}.
    \item \textit{Unreliable Wireless Connectivity}: Although 5G supports ultra-reliable low latency, service continuity remains challenging due to vehicle mobility and obstacle blockage \cite{Ameen_2019_deep}. In addition, the degradation of \gls{snr} in the wireless channel can cause a sudden breakdown in communication performance, which is known as the \textit{cliff effect}. 
    %It is the result of the binary nature of digital signals combined with the limitations of error correction techniques. 
    % \item \textbf{Robust Data Exchange}: Due to high data throughput, ensuring robust communication and data exchange with other vehicles, infrastructures, and cloud services is vital for informed decision-making \cite{Ameen_2019_deep}.
    \item \textit{Real-time Responsiveness and Latency}: Minimizing processing time for sensor data analysis and decision-making is crucial for timely response in edge-enabled autonomous driving \cite{Liu_2019_edge}.
    
\end{enumerate}
% How to address the challenges? The big picture here.
% new approach, bypass theoretical bond of shannon limitation, to improve the performance in the low snr region. support mission critical task in autonomous driving, we need a brand new approach, that is not limited by information theory.
%To cope with these challenges, a new framework that integrates communication and computing is urgently required. Furthermore, rethinking the boundary of the Shannol theory is critical to improve performance in the low \gls{snr} region. To support the mission-critical task in autonomous driving, we need a brand new approach, which is not limited by the information theory. 
To address challenges in connected autonomous systems, especially in low \gls{snr} environments, a paradigm shift that integrates communication with computing becomes essential. This shift drives rethinking the gap between bit-level transmission built upon Shannon's theory and the requirements of tasks in automation systems. Autonomous driving, as a mission-critical task, demands an innovative approach that extends communication efficiency beyond traditional information theory constraints.

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.90\linewidth]{Figure/general_idea.pdf}
    \end{center}
       \caption{Edge computing enabled autonomous driving.}
    \label{fig_general_idea}
\end{figure}

From the machine's perspective, high-fidelity reconstructions are often not needed, whereas mission-critical semantic information plays the most important role. Semantic communication, which has emerged as a fundamental aspect of 6G technologies, seeks to revolutionize this landscape by prioritizing data semantics over bit-level data transmission. In particular, \gls{jscc} integrates the entire transmission process for direct semantic transmission, contrasting traditional segmented considerations \cite{Chaccour_2022_less}. Deep learning enabled \gls{jscc} demonstrates resilience to the \textit{cliff effect}, showing superiority over separate source-channel coding, especially at lower \glspl{snr}, including the transmission of natural language \cite{Xie_2021_deep}, images \cite{Bourtsoulatze_2019_deep}, and videos \cite{Wang_2023_wireless}.

% What are the differences of our method? Others are not mission-critical
% the paragraph can be put into related work
% However, existing research mainly focuses on data-centric metrics (e.g., \gls{psnr}, \gls{msssim}) or basic tasks such as image classification \cite{Zhang_2023_deep}. Comprehensive applications utilizing deep \gls{jscc} for pragmatic tasks, particularly in autonomous driving, remain underexplored.

In this paper, we propose a novel deep \gls{tscc} framework based on modified \gls{cvae} to enhance edge-enabled autonomous driving. Inspired by \gls{jscc}-enabled image transmission \cite{Bourtsoulatze_2019_deep} and the integration of \gls{jscc} with \gls{vae} \cite{Saidutta_2021_joint}, our approach jointly designs data transmission with pragmatic tasks, building a resilient \gls{e2e} communication system against \gls{awgn}. Our methodology prioritizes task-oriented design, employing an \gls{e2e} autonomous driving agent as the metric for training deep \gls{jscc}. We innovatively integrate $\beta$-\gls{cvae} with the autonomous driving agent, offering a holistic view of task-oriented source-channel coding.

The major contributions of this work are summarised as follows:
\begin{itemize}
    \item We propose designing $\beta$-\gls{cvae} to synergize the autonomous driving agent with the source-channel coding, demonstrating a novel approach that integrates communications and computing in autonomous systems.
    \item By implementing \gls{tscc} within an edge-enabled state-of-the-art \gls{e2e} autonomous driving agent, we demonstrate notable improvements in driving performance over traditional communication methods and state-of-the-art deep \gls{jscc} approaches, particularly in terms of driving score.
    \item To the best of our knowledge, we pioneer the exploration of deep \gls{jscc} design for autonomous driving, illuminating the potential of comprehensive task-oriented deep \gls{jscc}.
    % framework jscc, imitation learning? 
\end{itemize}


==> _old/2_related_work.tex <==
\section{Related Work}
% JSCC
The rapid evolution of deep learning has catalyzed innovative communication designs, aiming to reach or even exceed the Shannon limit. Semantic communication, a prominent direction in this realm, emphasizes the semantics of data over the mere transmission of bits \cite{Chaccour_2022_less, Yang_2023_semantic, Qin_2022_semantic}. Deep \gls{jscc} emerges as a robust solution in different scenarios with limited bandwidth and low \glspl{snr}, which excels in task performance compared to traditional methods. In particular, in semantic communication, text transmission can sacrifice word fidelity for higher efficiency of utilization of communication resources, yet still conveys intended meanings \cite{Xie_2021_deep, Farsad_2018_deep}. Research in the deep \gls{jscc} for wireless image transmissions \cite{Kurka_2019_seccessive, Bourtsoulatze_2019_deep, Kurka_2020_deepJSCC} has demonstrated its superiority over traditional source coding (e.g., JPEG and JPEG2000) and channel coding (e.g., LDPC), especially in the low \gls{snr} region. However, existing research mainly focuses on data-centric metrics (e.g., \gls{psnr} \cite{Kurka_2019_seccessive, Tung_2022_deepJSCC, Yang_2022_OFDM, Tung_2022_deep, Kurka_2020_deepJSCC}, \gls{ssim} \cite{Bourtsoulatze_2019_deep, Tung_2022_deepJSCC, Yang_2022_OFDM, Kurka_2020_deepJSCC}, and \gls{msssim} \cite{Yang_2022_OFDM, Tung_2022_deep, Kurka_2020_deepJSCC}) to evaluate the effectiveness of deep \gls{jscc} design for image transmission. Although some basic tasks were explored with deep \gls{jscc}, such as image classification \cite{Zhang_2023_deep, Liu_2022_adaptable, Hu_2022_robust}, they were not developed for autonomous system communications. 
Mission-critical applications utilizing deep \gls{jscc} for pragmatic tasks, particularly in autonomous driving, remain underexplored.

The integration of deep \gls{jscc} into edge computing is a promising framework. \cite{Tung_2022_deepJSCC} proposed transmitting data through predefined constellations, which bridge the gap of applying deep \gls{jscc} to commercialize hardware and showcase the potential of deep \gls{jscc} in edge computing scenarios. The effectiveness of deep \gls{jscc} often depends on the conditions of the wireless channels, and thus the optimal solutions may change over the varying channel \glspl{snr}. The incorporation of \gls{vae} into the deep JSCC design \cite{Saidutta_2021_joint} has the potential to improve generalizability across different \glspl{snr}. Nevertheless, the effectiveness of this approach in autonomous systems remains unclear.

% Edge computing for autonomous driving
Autonomous driving requires massive volumes of data to process and poses significant challenges in terms of power constraints and communication latency \cite{Zhang_2020_mobile}. Traditional on-board processing and cloud computing struggle to meet these demands \cite{Zhang_2020_mobile}. Edge computing has emerged as a key solution in autonomous driving, and can meet the need for real-time data processing and decision making \cite{Liu_2019_edge}. Integration of edge computing with deep \gls{jscc} is a promising approach, which aims to achieve efficient semantic communication through task-oriented design. This combination is expected to enhance real-time analytics of sensor data, such as LiDAR data, radar data, and RGB images, paving the way for future advances in the field.

% Our work
The current literature reveals a gap in the application of deep \gls{jscc} in the context of edge computing for autonomous driving. Our research aims to bridge this gap by demonstrating how a deep \gls{jscc} (TSCC) framework, when implemented in an edge computing environment, can significantly improve the efficiency and reliability of data communication in autonomous vehicles. This approach not only improves data rates, but also ensures robust communications across various channel conditions, thereby fully utilizing the potential of autonomous vehicles in practical scenarios.



==> _old/3_system_model.tex <==
\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.9\linewidth]{Figure/case_study.pdf}
    \end{center}
       \caption{Framework of the \gls{tscc} enabled autonomous driving.}
    \label{fig_case_study}
\end{figure*}
\section{System Model}
The considered edge-enabled autonomous driving scenario is shown in \cref{fig_general_idea}. 
%An automated vehicle with a variety of sensors, such as RGB cameras, depth cameras, LiDARs, radars, and speedometers, is connected to the edge server. 
In our case study, we consider an automated vehicle equipped with a single RGB camera on the front, which is connected to the edge server. Sensor data are encoded and transmitted to the edge server via wireless communications, where the edge server, located at a base station, serves as a computational hub. The data are processed by an autonomous driving agent, deployed at the edge server, interpreting the information and generating appropriate control commands for the vehicle's current scenario. These commands are transmitted back to the vehicle for safe autonomous driving. Since the agent makes decisions based on the images obtained from the RGB camera, image compression and transmission are critical to the performance of the edge-enabled autonomous driving system.

%Traditional data compression methods in communication systems, such as quantization, entropy coding, and lossy compression algorithms, aim to minimize bit rates at a certain distortion level. These methods did not consider the semantics of the data, leading to suboptimal task performance, particularly at low \glspl{snr}.

%Semantic-based compression methods focus on capturing the most semantically relevant features of the data, offering robustness against transmission errors in low SNR scenarios. Nevertheless, for complex mission-critical systems like autonomous vehicles, considering data semantics alone may not suffice. Therefore, we propose a shift towards task-oriented communications, focusing on the end goal of the communication system and integrating the specific task requirements and goals of the autonomous driving system.

%This task-oriented approach promises to enhance communication effectiveness, potentially outperforming traditional and semantic-based methods in challenging conditions. 
The following sections present a case study demonstrating our proposed \gls{tscc}'s implementation and effectiveness in edge-enabled autonomous driving, which focuses on bandwidth utilization and noise resistance for image transmission. We demonstrate the loss function and the training process, using an \gls{e2e} autonomous driving framework based on a monocular RGB camera as a baseline. \Cref{fig_case_study} illustrates our case study implementation, providing a practical perspective on the theoretical concepts. In particular, our approach integrates deep \gls{jscc} within the edge computing framework to address the challenges of bandwidth constraint and data transmission efficiency. 

\subsection{Variational Autoencoder}
\glspl{vae} \cite{VAE} are a class of generative models that leverage the power of neural networks for the encoding and decoding process while incorporating a probability distribution for data generation and latent space modeling. The system model comprises two neural networks: an encoder $q_{\phi}(\bm{z}\mid \bm{x})$ with parameters $\phi$, and a decoder $p_{\theta}(\bm{x}\mid \bm{z})$ with parameters $\theta$. The encoder transforms the data sample $\bm{x}$ into latent vector $\bm{z}$, while the decoder reconstructs the original data from the latent vector.

%It consists of two neural networks: an encoder $q_{\phi}(\bm{z}\mid \bm{x})$, where $\phi$ is the parameters of the neural network, to encode a data sample $\bm{x}$ to latent vector $\bm{z}$ and a decoder $p_{\theta}(\bm{x}\mid \bm{z})$, where $\theta$ is the parameters of the neural network, to decode the latent vector to original data space. 
%Given an input data sample $\bm{x}$, the encoder neural network $q_{\phi}(\bm{z}\mid \bm{x})$, where $\phi$ is the parameters of the neural network, maps it to a distribution over the latent space, where a vector $\bm{z}$ in the latent space is typically imposed a prior $\bm{z} \sim \mathcal{N}(\bm{0}, \mathbf{I})$. A latent vector $\bm{z}$ is then sampled by \textit{reparameterization trick} to maintain the differentiability, which is essential for backpropagation during training.

%This sampled latent vector $\bm{z}$ is fed into the decoder neural network $p_{\theta}(\bm{x}\mid \bm{z})$, where $\theta$ is the parameters of the neural network, which attempts to reconstruct the original data sample $\bm{x}$. 
The training of \gls{vae} is to minimize the following loss function:
\begin{align}
\mathcal{L}_\text{VAE}(\bm{x}; \phi, \theta)
    %= & -\text{ELBO}(\bm{x}) \label{eq_loss_vae_1}\\
    = & \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x})}\left[-\ln p_{\theta}(\bm{x} \mid \bm{z})\right] \notag\\
    & + \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x})}\left[\ln{\frac{q_{\phi}(\bm{z} \mid \bm{x})}{p(\bm{z})}}\right]  \label{eq_loss_vae_2}\\
    = & \frac{1}{t} \sum_{i=1}^{t}\Vert \bm{x} - \hat{\bm{x}}_{i} \Vert^{2} \notag \\ 
    & + \frac{1}{2}\sum_{j=1}^{d}(\mu_{j}^{2}+\sigma_{j}^{2} - \ln\sigma_{j}^{2} - 1) \label{eq_loss_vae_details}\\
    = & \mathcal{L}_{\text{rec}}(\bm{x}; \phi, \theta) + \mathcal{L}_{\text{KL}}(\bm{x}; \phi) \label{eq_loss_vae_3}.
\end{align}
\Cref{eq_loss_vae_details} assumes that $p_{\theta}(\bm{x}\mid\bm{z})$ follows a Gaussian distribution with constant standard deviation \cite{Pytorch_VAE}. The reconstructed data $\hat{\bm{x}}_{i}$ is derived from the decoder $p_{\theta}(\bm{x}\mid \bm{z}_{i})$, and $t$ represents the number of latent vectors sampled from the latent space. The latent vector, $\bm{z} \in \mathbb{R}^{d}$, follows the Gaussian distribution with mean $\bm{\mu} \in \mathbb{R}^{d}$ and standard deviation $\bm{\sigma} \in \mathbb{R}^{d}$, where $d$ denotes the dimension of the latent space. 
$\mathcal{L}_{\text{rec}}(\bm{x}; \phi, \theta)$ is the first term in \cref{eq_loss_vae_details}, which represents the reconstruction errors. Meanwhile, $\mathcal{L}_{\text{KL}}(\bm{x}; \phi)$ is the second term in \cref{eq_loss_vae_details}, which represents the Kullback-Leibler (KL) divergence. In addition, the prior distribution $p(\bm{z})$ is assumed to be a standard Gaussian distribution $\mathcal{N}(\bm{0}, \mathbf{I})$.


$\beta$-\gls{vae} \cite{beta_VAE} extended the loss function of vanilla \gls{vae} by adding an coefficient $\beta_{\text{rec}}$:
\begin{equation}
    \mathcal{L}_\text{VAE}(\bm{x}; \phi, \theta)
    = \beta_{\text{rec}}\mathcal{L}_{\text{rec}}(\bm{x}; \phi, \theta) + \mathcal{L}_{\text{KL}}(\bm{x}; \phi),
    \label{eq_loss_betaVAE}
\end{equation}
where $\beta_{\text{rec}}$ for $\mathcal{L}_{\text{rec}}(\bm{x}; \phi, \theta)$ to control the training balance.

\Gls{cvae} introduces a class label $m$ as a condition, with which the new loss function can be extended in the following expression:
\begin{align}
    \mathcal{L}_{\text{CVAE}}(\bm{x}, \bm{m}; \phi, \theta) = & \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x}, \bm{m})}\left[-\ln p_{\theta}(\bm{x} | \bm{z}, \bm{m})\right] \notag \\ 
    & + \mathbb{E}_{\bm{z} \sim q_{\phi}(\bm{z} \mid \bm{x}, \bm{m})}\left[\ln{\frac{q_{\phi}(\bm{z} | \bm{x}, \bm{m})}{p(\bm{z} | \bm{m})}}\right]  \\
    = & \frac{1}{t} \sum_{i=1}^{t}\Vert \bm{x} - \hat{\bm{x}}_{i} \Vert^{2} \notag \\ 
    & + \frac{1}{2}\sum_{i=1}^{d}(\mu_{i}^{2}+\sigma_{i}^{2} - \ln\sigma_{i}^{2} - 1) \label{eq_loss_cvae_details}\\
    = & \mathcal{L}_{\text{c-rec}}(\bm{x}, \bm{m}; \phi, \theta) + \mathcal{L}_{\text{c-KL}}(\bm{x}, \bm{m}; \phi).
    \label{eq_loss_cvae}
\end{align}

The autoencoder has been used to train deep \gls{jscc} in an \gls{e2e} manner \cite{Xie_2021_deep, Weng_2021_semantic, Saidutta_2021_joint}. Inspired by \cite{Saidutta_2021_joint}, we designed \gls{tscc} based on $\beta$-\gls{cvae}.

\subsection{Onboard Image Processing}
\label{subsec_sysMod_framework}
The input RGB image is denoted by $\bm{x} \in \mathbb{R}^{l}$, where $l = C\times H \times W$ is defined as the source bandwidth \cite{Bourtsoulatze_2019_deep}. $C$ stands for the number of color channels in the image. 
%For RGB images, there are three channels (red, green, and blue). 
$H$ and $W$ represent the height and width of the image, respectively, measured in pixels.

On the vehicle side, instead of directly mapping RGB images to channel inputs \cite{Bourtsoulatze_2019_deep}, we first obtain the distribution of the latent vector from the encoder,
\begin{equation}
    (\bm{\mu}, \bm{\sigma}) = \mathrm{T}_\alpha(\bm{x}),
    \label{eq_task_encoder}
\end{equation}
where $\mathrm{T}_\alpha(\cdot)$ is the joint task encoder with the parameters $\alpha$. The encoder outputs the mean $\bm{\mu}$ and the standard deviation $\bm{\sigma}$ of the latent vector. 
The latent vector $\bm{z}$ is sampled by the \textit{reparameterization trick}
\begin{align}
    \bm{z} = \bm{\epsilon}\odot \bm{\sigma} + \bm{\mu},
    \label{eq_reparam}
\end{align}
where $\bm{\epsilon} \in \mathbb{R}^{d}$ is sampled from $\mathcal{N}(\bm{0}, \mathbf{I})$, $\odot$ is elements-wise multiplication. The channel inputs $\check{\bm{z}} \in \mathbb{C}^{k}$ can be obtained from the latent vector $\bm{z}$ by combining every two neighboring elements into a single complex number. The dimension of the complex vector is half of the original latent vector, $k=d/2$. This operation is represented by a reshaping function,
\begin{align}
    \check{\bm{z}} = \mathrm{F}(\bm{z}).
    \label{eq_reshape}
\end{align}
To ensure that the channel inputs $\tilde{\bm{z}}$ satisfied the power constraint $\frac{1}{k}\mathbb{E}\| \tilde{\bm{z}}\|^{2}\leq P$, where $P$ is the average transmit power constraint, $\check{\bm{z}}$ is normalized as:
\begin{align}
    \tilde{\bm{z}} = \mathrm{N}(\check{\bm{z}}) \triangleq \sqrt{kP}\frac{\check{\bm{z}}}{\sqrt{\check{\bm{z}}^{*}\check{\bm{z}}}},
    \label{eq_norm_details}
\end{align}
where $\mathrm{N}(\cdot)$ denotes the normalization function, $\tilde{\bm{z}}^{*}$ is the conjugate transpose of $\tilde{\bm{z}}$.
In the case of $k<l$, we define ${k}/{l}$ as the \textit{compression ratio} \cite{Bourtsoulatze_2019_deep}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
The channel output is given by 
\begin{equation}
    \hat{\bm{z}} = \bm{h}\odot \bm{z}+\bm{n},
    \label{eq_channel_layer}
\end{equation}
where $\bm{n} \sim \mathcal{CN}(0, \bm{\sigma}_{\mathrm{awgn}}^{2}\mathbf{I})$, $\bm{h} \in \mathbb{C}^{k}$ is the channel fading coefficient for the Rayleigh fading channel $\mathcal{CN}(\bm{0}, \mathbf{I})$. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For the \gls{awgn} channel, the channel output can be given as follows,
\begin{equation}
    \hat{\bm{z}} = \tilde{\bm{z}}+\bm{n},
\end{equation}
where $\hat{\bm{z}}$ is received channel inputs. 
The reconstructed image $\bm{y}$ can be obtained from the decoder, i.e.,
\begin{equation}
    \bm{y} = \mathrm{T}^{-1}_\delta(\mathrm{F}^{-1}(\hat{\bm{z}})),
    \label{eq_task_decoder}
\end{equation}
where $\mathrm{T}^{-1}_\delta(\cdot)$ is the task decoder with parameters $\delta$, and $\mathrm{F}^{-1}$ is the inverse reshaping function. 

Since the goal of our task-oriented design is to maximize autonomous driving performance rather than to minimize the difference between $\bm{x}$ and $\bm{y}$, the loss function should preserve the most task-relevant information for the autonomous driving agent and take driving performance into account as the optimization target.

\subsection{Edge-Enabled Autonomous Driving Agent}
In autonomous driving scenarios, accurate control commands are crucial and rely on environmental data (e.g., RGB images) and state information (including navigation information, vehicle speed, throttle, brake, and steering angle). As depicted in \cref{fig_case_study}, this state information, denoted by $\bm{m}$, is transmitted using traditional communication methods for two main reasons: 1) semantic communication may not guarantee the fidelity required for critical information; 2) the required data rate for the transmission of state information is very low.
%3) our initial research focuses on the application of \gls{jscc} for image transmission in edge-enabled autonomous driving environments.

Upon receiving state information $\hat{\bm{m}}$ and the reconstructed image $\bm{y}$, the edge-deployed autonomous driving agent generates control commands as follows:
\begin{equation}
    \hat{\bm{a}} = \mathrm{A}_{\psi}(\bm{y}, \hat{\bm{m}}),
\end{equation}
where $\mathrm{A}_{\psi}$ represents the autonomous driving agent, and $\hat{\bm{a}}$ are the control commands derived from the received information. In particular, we assume $\bm{m}=\hat{\bm{m}}$ in this case study.

\subsection{Training of Task-Oriented CVAE}
% This part needs to be thought carefully.
Baseline control commands $\bm{a}$ are produced by a coach AI \cite{Roach} using lossless images and state information.
%Assuming that there exists a very deep neural network mapping $(\bm{a}, \bm{m})$ to $\bm{x}$, denoted as $\bm{x} = \mathrm{G}_{\xi}(\bm{a}, \bm{m})$, where $\xi$ is parameters of neural network, 
We design the $\beta$-\gls{cvae} for the mapping from $\bm{a}$ to $\hat{\bm{a}}$. Combining \cref{eq_loss_betaVAE}, \cref{eq_loss_cvae_details}, and \cref{eq_loss_cvae}, we design the task-oriented loss function of \gls{tscc} as
\begin{align}
    \mathcal{L}_{\text{TSCC}}(\bm{a}, \bm{m}; \alpha, \delta)= & \beta_{\text{c-rec}}\mathbb{E}_{\bm{z} \sim q_{\alpha}(\bm{z} \mid \bm{a}, \bm{m})}[-\ln p_{\delta}(\bm{a} | \bm{z}, \bm{m})] \notag \\
    & + \mathbb{E}_{\bm{z} \sim q_{\alpha}(\bm{z} \mid \bm{a}, \bm{m})}\left[\ln{\frac{q_{\alpha}(\bm{z} | \bm{a}, \bm{m})}{p(\bm{z} | \bm{m})}}\right]\\
    = & \beta_{\text{c-rec}}\frac{1}{t} \sum_{i=1}^{t}\Vert \bm{a} - \hat{\bm{a}}_{i} \Vert^{2} \notag \\ 
    & + \frac{1}{2}\sum_{i=1}^{d}(\mu_{i}^{2}+\sigma_{i}^{2} - \ln\sigma_{i}^{2} - 1)\\
    = & \beta_{\text{c-rec}} \mathcal{L}_{\text{c-rec}}(\bm{a}, \bm{m}; \alpha, \delta) \notag \\
    &+ \mathcal{L}_{\text{c-KL}}(\bm{a}, \bm{m}; \alpha).
\end{align}
The first term $\mathcal{L}_{\text{c-rec}}(\cdot)$ ensures the fidelity of actions $\hat{\bm{a}}$ under the given state information $\bm{m}$. Meanwhile, the second term $\mathcal{L}_{\text{c-KL}}(\cdot)$ is adversarial to the first term $\mathcal{L}_{\text{c-rec}}(\cdot)$, and introduces noise into the training process. Since $\mathcal{L}_{\text{c-KL}}$ introduces noise, we can train \gls{tscc} without channel noise and execute \gls{tscc} over practical channels with various \glspl{snr}. Furthermore, the hyperparameter $\beta_{\text{c-rec}}$ balances two terms to achieve a good trade-off between action fidelity and noise-resistant ability.
The training process of the proposed \gls{tscc} is shown in \cref{alg_cvae_train}.

\input{Algrithm/alg_cvae_train}

%Importantly, maintaining the structure and parameters of the autonomous driving agent intact is not trivial. With minimal modifications, the same agent can be deployed at both the edge and the vehicle, demonstrating substantial potential for generalization across various autonomous driving scenarios.


==> _old/4_result.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.7\linewidth]{Figure/bandComp.pdf}
    \end{center}
       \caption{Driving score of traditional image coding method with varied compression ratio.}
    \label{fig_bandComp}
\end{figure}
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.7\linewidth]{Figure/results.pdf}
    \end{center}
       \caption{Driving score with varied \gls{snr}.}
    \label{fig_results}
\end{figure}
\section{Simulation Result}
\subsection{Dataset}
CARLA is an open-source simulator \cite{CARLA}, which offers diverse urban environments to facilitate research on autonomous driving.
%An open-source simulator, CARLA, to provide diverse urban environments for autonomous driving as in \cite{CARLA}. 
It offers dynamic agents and traffic scenarios as in real-world driving conditions. The image dataset from \cite{Wu_2022_TCP} is used to train \gls{tscc}. This dataset comprises images ($C=3$, $H=256$, and $W=900$) across various urban maps, with training and testing sets containing 189,524 (four maps: Town01, Town03, Town04, and Town06) and 27,201 images (four maps: Town02, Town05, Town07, and Town10), respectively. In addition to offline image testing, we use Town05 to test our proposed framework in real time.

\subsection{Evaluation Metrics}
To evaluate the effectiveness of our approach, we compare the driving performance of \gls{tscc} with different baselines in the CARLA simulator. The driving score\footnote{\url{https://leaderboard.carla.org/}} has been widely used in the existing literature to evaluate the vehicle's ability to follow predetermined waypoints, reach the destination, and avoid violating traffic rules. The tests are carried out in \textbf{Town05} with four different scenarios (clear noon, cloudy sunset, soft rain down, and hard rain night), where the test is repeated three times in each scenario. 
%Driving performance can be evaluated in three aspects: route completion score, infraction score, and driving score\footnote{\url{https://leaderboard.carla.org/}}. The route completion score quantifies the ratio of completed road segments to the total planned distance; the infraction score takes into account any rule violations initiated by the autonomous agent; and the overall driving score, based on the previous two metrics, is an indicator of overall performance.

\subsection{Evaluation on CARLA}
The impacts of the compression ratio on the driving score are shown in \cref{fig_bandComp}. We compare our approach with traditional image coding methods: JPEG, JPEG2000, and BPG. The source (image) coding is followed by (2048, 6144) LDPC codes with 64-QAM digital modulation schemes. Specifically, their compression ratios range from 0.009 to 0.251.
For the proposed \gls{tscc} neural network, we set $d=4096$ and $k=2048$, resulting in a significantly lower compression ratio $k/l$ of 0.003. In addition, we set $\beta_{\text{c-rec}}=2048$ and $P=1$. The results show that when the required driving score is 20, the \gls{tscc} framework could save 98.36\% communication bandwidth compared to the existing methods.

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.8\linewidth]{Figure/qualitative_result.pdf}
    \end{center}
       \caption{Qualitative example of \gls{tscc} and baseline methods at 10 dB \gls{snr}. The compression ratios of example images are shown in the lower right corner.}
    \label{fig_qualitative}
\end{figure}

\input{Table/tradi_metrics}

As shown in \cref{fig_results}, the driving score highly depends on \gls{snr}. The compression ratios of JPEG, JPEG2000, and BPG are set to 0.232, 0.251, and 0.183, respectively. The compression ratio of our method is set to 0.003. In addition, we compare the proposed \gls{tscc} with the state-of-the-art \gls{jscc} method using the same neural network structure, with legends ``JSCC-AE'' \cite{Bourtsoulatze_2019_deep} and ``JSCC-VAE'' \cite{Saidutta_2021_joint}. We trained JSCC-AE with different \glspl{snr} and found that the testing performance is similar. In this figure, JSCC-AE is trained with 0 dB \gls{snr}. Like the training of \gls{tscc}, JSCC-VAE is trained without channel noise.

The results show that our \gls{tscc} achieves much higher driving scores at 0 dB \gls{snr} (19.82) and -5 dB \gls{snr} (14.5), respectively, compared to other methods. In contrast, the driving scores of traditional image coding methods drop dramatically in the low \gls{snr} region (below 0 dB). 
%\textcolor{red}{Meanwhile, JSCC-VAE and JSCC-AE show noise resistance ability and good perceptual quality for human vision, but they fail to preserve mission-critical information, such as road marks and pedestrians, leading to poor performance for edge-enabled autonomous driving.}

Although traditional image coding, JSCC-AE, and JSCC-VAE yield high-quality image reconstructions for human vision, as shown in \cref{fig_qualitative}, they retain redundant information not critical to machine vision. In particular, some mission-critical information, such as pedestrians and road markers, is not clearly presented by JSCC-AE and JSCC-VAE, leading to poor performance for edge-enabled autonomous driving. In \cref{tab_tradi_metrics}, we evaluate some other performance metrics, including \gls{psnr}, \gls{msssim}, and \gls{fid}, which are specially designed for human perception. The different preferences between human vision and machine vision indicate the importance of task-oriented source-channel coding design for machine vision. 
%and the lack of mission-critical guidance in traditional human perceptual metrics.


==> _old/5_conclusion.tex <==
\section{Conclusion}
We proposed a \gls{tscc} framework for edge-enabled autonomous driving that takes advantage of the knowledge of a well-trained autonomous driving agent. We designed $\beta$-\gls{cvae} in a task-oriented way to guide the training of deep source-channel coding to preserve mission-critical information for machine vision. We carried out a case study in CARLA and the results showed that proposed \gls{tscc} save 98.36\% communication bandwidth compared with the existing method when \gls{snr} is 10 dB. In the low \gls{snr} region (below 0 dB), all traditional methods and existing \gls{jscc} approaches do not work, while our \gls{tscc} approach can still achieve 83.24\% or 60.9\% driving scores when \gls{snr} is 0 dB or -5 dB.

